Shuffled Patch-Wise Supervision for Presentation Attack Detection

Face anti-spoofing is essential to prevent false facial verification by using a photo, video, mask, or a different substitute for an authorized person's face. Most of the state-of-the-art presentation attack detection (PAD) systems suffer from overfitting, where they achieve near-perfect scores on a single dataset but fail on a different dataset with more realistic data. This problem drives researchers to develop models that perform well under real-world conditions. This is an especially challenging problem for frame-based presentation attack detection systems that use convolutional neural networks (CNN). To this end, we propose a new PAD approach, which combines pixel-wise binary supervision with patch-based CNN. We believe that training a CNN with face patches allows the model to distinguish spoofs without learning background or dataset-specific traces. We tested the proposed method both on the standard benchmark datasets -- Replay-Mobile, OULU-NPU -- and on a real-world dataset. The proposed approach shows its superiority on challenging experimental setups. Namely, it achieves higher performance on OULU-NPU protocol 3, 4 and on inter-dataset real-world experiments.

==> tables/cross_dataset.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|} 
\hline
                             & \multicolumn{2}{c|}{\textbf{Trained on OULU}}                           & \multicolumn{2}{c|}{\textbf{Trained on RM}}                              \\ 
\hline
\textbf{Model}               & \multicolumn{1}{l|}{tested on OULU} & \multicolumn{1}{l|}{tested on RM} & \multicolumn{1}{l|}{tested on OULU} & \multicolumn{1}{l|}{tested on RM}  \\ 
\hline
IQM-SVM                      & 24.6                                & 31.6                              & \textbf{3.9}                        & 42.3                               \\
LBP-SVM                      & 32.2                                & 35.0                              & 12.1                                & 43.6                               \\
DeepPixBis                   & \textbf{0.4}                        & 12.4                              & 22.7                                & \textbf{0.0}                       \\
\textbf{Ours (DenseNet)}     & 2.14                                     & 29.90                                   & 28.61                                     & 0.0                                \\
\textbf{Ours (EfficientNet)} & 2.56                                     & 22.82                                   & 32.57                                     & 0.0                                \\
\hline
\end{tabular}
\caption{Inter-dataset testing results of OULU-NPU (Protocol 1) and Replay-Mobile (grandtest) protocol. Reported metrics in the table represents the HTER values in percentage(\%)}
\end{table}

==> tables/oulu_table_old.tex <==
\begin{table}
\begin{tabular}{|c|c|c|c|c|} 
\hline
\textbf{Protocol}                        & \textbf{Model}       & \textbf{APCER(\%)}   & \textbf{BPCER(\%)}   & \textbf{ACER(\%)}     \\ 
\hline
\multicolumn{1}{|c|}{\multirow{8}{*}{1}} & GRADIANT             & 1.3                  & 12.5                 & 6.9                   \\
\multicolumn{1}{|c|}{}                   & FAS-BAS              & 1.6                  & 1.6                  & 1.6                   \\
\multicolumn{1}{|c|}{}                   & LBP-SVM              & 12.92                & 51.67                & 32.29                 \\
\multicolumn{1}{|c|}{}                   & \textbf{CDCN}        & \textbf{0.4}         & 1.7                  & 1.0                   \\
\multicolumn{1}{|c|}{}                   & \textbf{CDCN++}      & \textbf{0.4}         & \textbf{0.0}         & \textbf{0.2}          \\
\multicolumn{1}{|c|}{}                   & \textbf{DeepPixBis}  & 0.83                 & \textbf{0.0}         & 0.42                  \\
\multicolumn{1}{|c|}{}                   & Ours(DenseNet)       & 2.14                 & 2.14                 & 2.14                      \\
\multicolumn{1}{|c|}{}                   & Ours(EfficientNet)   & 2.54                   & 2.58              & 2.56                      \\ 
\hline
\multicolumn{1}{|c|}{\multirow{8}{*}{2}} & GRADIANT             & 3.1                  & 1.9                  & 2.5                   \\
                                         & FAS-BAS              & 2.7                  & 2.7                  & 2.7                   \\
                                         & LBP-SVM              & 30                   & 20.28                & 25.14                 \\
                                         & \textbf{CDCN}        & \textbf{1.5}         & 1.4                  & 1.5                   \\
                                         & \textbf{CDCN++}      & 1.8                  & \textbf{0.8}         & \textbf{1.3}          \\
                                         & DeepPixBis           & 11.39                & 0.56                 & 5.97                  \\
                                         & Ours(DenseNet)       & 6.22                 & 6.26                 & 6.24                       \\
                                         & Ours(EfficientNet)   & 5.10                 & 5.89                 & 5.49                      \\ 
\hline
\multicolumn{1}{|c|}{\multirow{8}{*}{3}} &  GRADIANT             & $2.6\pm3.9$          & $5.0 \pm 5.3$        & $3.8 \pm 2.4$         \\
                                         & FAS-BAS              & $2.7\pm1.3$          & $3.1\pm1.7$          & $2.9\pm1.5$           \\
                                         & LBP-SVM              & $28.5\pm23.05$       & $23.33\pm17.98$      & $25.92\pm11.25$       \\
                                         & CDCN                 & $2.4\pm1.3$          & $2.2\pm2.0$          & $2.3\pm1.4$           \\
                                         & \textbf{CDCN++}      & \textbf{$1.7\pm1.5$} & \textbf{$2.0\pm1.2$} & \textbf{$1.8\pm0.7$}  \\
                                         & DeepPixBis           & $11.67\pm19.57$      & $10.56\pm14.06$      & $11.11\pm9.4$         \\
                                         & Ours(DenseNet)       & $6.10\pm2.57$        & $6.30\pm2.55$        & $6.20\pm2.55$                 \\
                                         & Ours(EfficientNet)   & $\pm$                & $\pm$                & $\pm$                 \\ 
\hline
\multicolumn{1}{|c|}{\multirow{8}{*}{4}} &  GRADIANT             & $5.0\pm4.5$          & $15.0\pm7.1$         & $10.0\pm5.0$          \\
                                         & FAS-BAS              & $9.3\pm5.6$          & $10.4\pm6.0$         & $9.5\pm6.0$           \\
                                         & LBP-SVM              & $41.67\pm27.03$      & $55.0\pm21.21$       & $48.33\pm6.07$        \\
                                         & CDCN                 & $4.6\pm4.6$          & $9.2\pm8.0$          & $6.9\pm2.9$           \\
                                         & \textbf{CDCN++}      & \textbf{$4.2\pm3.4$} & \textbf{$5.8\pm4.9$} & \textbf{$5.0\pm2.9$}  \\
                                         & DeepPixBis           & $36.67\pm29.67$      & $13.33\pm16.75$      & $25.0\pm12.0$         \\
                                         & Ours(DenseNet)       & $11.51\pm7.86$                & $11.58\pm7.84$                & $11.54\pm7.84$                 \\
                                         & Ours(EfficientNet)   & $\pm$                & $\pm$                & $\pm$                 \\ 
\hline
\end{tabular}
\caption{Intra-dataset test results of OULU-NPU dataset}
\end{table}
